MeLPUF: Memory-in-Logic PUF Structures for Low-Overhead IC Authentication

Physically Unclonable Functions (PUFs) are used for securing electronic devices across the implementation spectrum ranging from Field Programmable Gate Array (FPGA) to system on chips (SoCs). However, existing PUF implementations often suffer from one or more significant deficiencies: (1) significant design overhead; (2) difficulty to configure and integrate based on application-specific requirements; (3) vulnerability to model-building attacks; and (4) spatial locality to a specific region of a chip. These factors limit their application in the authentication of designs used in diverse applications. In this work, we propose MeLPUF: Memory-in-Logic PUF; a low-overhead, distributed PUF that leverages the existing logic gates in a design to create cross-coupled inverters (i.e., memory cells) in a logic circuit as an entropy source. It exploits these memory cells' power-up states as the entropy source to generate device-specific unique fingerprints. A dedicated control signal governs these on-demand memory cells. They can be dispersed across the combinational logic of a design to achieve distributed authentication. They can also be synthesized with a standard logic synthesis tool to meet the target area, power, and performance constraints. We evaluate the quality of MeLPUF signatures with circuit-level simulations and experimental measurements using FPGA silicon (TSMC 55nm process). Our analysis shows the high quality of the PUF in terms of uniqueness, randomness, and robustness while incurring modest overhead. We further demonstrate the scalability of MeLPUF by aggregating power-up states from multiple memory cells, thus creating PUF signatures or digital identifiers of varying lengths. Additionally, we suggest optimization techniques that can be leveraged to boost the performance of MeLPUF further.

==> sections/Related_Work.tex <==
\subsection{Related Work}


==> sections/Synthesis.tex <==

\section{MeLPUF Integration}
\label{sec:synthesis}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=3.25in,height=5.25in,keepaspectratio]{fig/FlowChart.png}
%\caption{MeLPUF synthesis tool flowchart.}
%\label{fig:flow}
%\vspace{-10pt}
%\end{figure}

%Figure~\ref{fig:flow} describes the various steps involved in synthesizing a MeLPUF based design. The MeLPUF synthesis flow takes as inputs the design represented in a high-level language such as Verilog, Chisel or VHDL or as a set of gates synthesized using a standard cell library. The standard cell library contains the set of gates provided by the foundry, the number of MeLPUFs to be inserted, and the set of inverter instances available in the standard cell library. The user also has the option to indicate whether the input netlist is synthesized or unsynthesized by using the \texttt{synthesized} flag.
%
%    \begin{figure}[!t]
%    \centering
%   \includegraphics[width=0.8\columnwidth]{fig/LUTMeL.png}
%    \caption{MeLPUF implementation on multiple LABs }
%    \label{fig:LUT}
%    \vspace{-15pt}
%\end{figure}
%
%
%The synthesis tool first parses the user arguments and checks for the \texttt{synthesized} flag. If the flag is not set, the tool synthesizes the netlist and converts the high-level representation into the set of corresponding gates. The tool then identifies the inverters present in the design by using the inverter instances provided as an input. The standard cell library typically contains multiple instances of an inverter characterized by various performance and power constraints. The user can provide all or a subset of these instances. The tool marks all the occurrences of the inverters in the synthesized netlist. The tool then selects a subset of these inverters and replaces them with the MeLPUF structure shown in Figure~\ref{fig:LUT}. The number of inverters selected is equal to the number of MeLPUF instances that the user wants to be inserted into the design. Once the insertion process is complete, the tool generates the area, power, and timing overheads.



  
% \end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Using multiple PUFs as a way to thwart machine learning attacks has been proposed in \cite{bib:mac}. Similarly, this distributed nature of the PUF makes model-building attacks more difficult to succeed. Additionally, it is also likely to make potential tampering of PUFs more difficult by an untrusted entity. Finally, it allows each IP to have a unique Silicon identifier, enabling us to track-and-trace and ``meter’’ each instance of an IP in fabricated SoC instances. This approach ensures that the SoC signature represents each IP component. If any issue such as tampering arises in an IP block that will cause its authentication signature to fail the individual IP can be identified and addressed as needed. Compared to watermarks, which provides a potentially clonable signature of an IP, such distributed PUFs allow unique unclonable identifier for each Silicon instance of an IP in fabricated SoCs. 







==> sections/abstract.tex <==
\begin{abstract}

Physical Unclonable Functions (PUFs) are used for securing electronic devices across the implementation spectrum ranging from Field Programmable Gate Array (FPGA) to system on chips (SoCs). However, existing PUF implementations often suffer from one or more significant deficiencies: (1) significant design overhead; (2) difficulty to configure and integrate based on application-specific requirements; (3) vulnerability to model-building attacks; and (4) spatial locality to a specific region of a chip. These factors limit their application in the authentication of designs used in diverse applications. In this work, we propose~\melpuf~: Memory-in-Logic PUF; a low-overhead, distributed PUF that leverages the existing logic gates in a design to create cross-coupled inverters (\emph{i.e.}, memory cells), in a logic circuit as an entropy source. It exploits these memory cells' power-up states as the source of entropy to generate device-specific unique fingerprints. A dedicated control signal governs these on-demand memory cells. They can be dispersed across the combinational logic of a design to achieve distributed authentication. They can also be synthesized with a standard logic synthesis tool to meet the target area, power, and performance constraints. We evaluate the quality of \melpuf~~signatures with circuit-level simulations and experimental measurements using  FPGA silicon (TSMC 55nm process). Our analysis shows the high quality of the PUF in terms of uniqueness, randomness, and robustness while incurring modest overhead. We further demonstrate the scalability of \melpuf~ by aggregating power-up states from multiple memory cells, thus creating PUF signatures or digital identifiers of varying lengths. Additionally, we suggest optimization techniques that can be leveraged to boost the performance of \melpuf~~further.

\end{abstract}

==> sections/algorithm.tex <==
\subsection{Synthesis algorithm and tool}

\begin{figure}[!h]
\centering
\includegraphics[width=2.5in]{fig/puf_synth_flowchart.jpg}
\caption{\melpuf synthesis tool flowchart.}
\label{fig:sysex}
\end{figure}

The \melpuf can be inserted in a provided design with the help of a tool. The tools accepts configuration parameters through a configuration file, the parameters being - design file, technology library, number of \melpuf to be inserted, inverter cell name(to target inverter cells to be replaced in the design file), etc. The input design file can be both synthesized or unsynthesized, but a synthesized design file have to follow certain naming conventions. The tool next identifies the cell name of the inverter but in case a input design uses multiple inverter cells it is recommended that a target inverter cell type is provided, and identifies all of that cell type in the input design file. The required number of inverters - equal to the number of \melpuf is randomly selected from the all of the identified invereter cells from the input design file and replace with \melpuf structure(Fig. 1). Finally reports - area, power and timing are generated for both the original and the \melpuf synthesized design and the overhead caused is reported for user review.

==> sections/experimental.tex <==
\subsection{Experimental Measurements}
    


==> sections/keywords.tex <==
\begin{IEEEkeywords}
distributed authentication, PUF, FPGA, SoC, CRP,  modeling attack, uniqueness, robustness, randomness.
\end{IEEEkeywords}

==> sections/method1.tex <==
\section{System on Chip Protection Methodology}
\label{sec:socprotect}
In This section, we illustrate that the distributed nature of~\melpuf~ can be used to secure a 
System on Chip (SoC).

\subsection{Gate Identification}
\label{sec:gates}
The first step is to identify the right set of gates for inserting the \melpuf~ structure. 
The inserted structure has a bistable circuit comprising of two cross-coupled inverters and control logic for reading the value. Upon powering on, the values at the two inverter inputs are randomly initialized due to which they enter a meta-stable state. The value at the output stabilizes to either a 1 or a 0 at random. The control signal can be used to read the value of the bi-stable element. Fig.~\ref{fig:sy2} shows the proposed \melpuf~~structure integrated into a digital design. To the best of our knowledge \melpuf~ is the first fully synthesizable PUF structure. 



==> sections/obsolete_references.tex <==
\begin{thebibliography}{1}

\bibitem{bib:model}
U. Rührmair, J. Sölter, F. Sehnke, X. Xu, A. Mahmoud, V. Stoyanova, et al., \emph{PUF modeling attacks on simulated and silicon data}, IEEE Transactions on Information Forensic and Security, vol. 8, pp. 1876-1891, 2013.

\bibitem{bib:proper}
R. Maes and I. Verbauwhede, \emph{Physically Unclonable Functions: A Study on the State of the Art and Future Research Directions,} in Towards Hardware-Intrinsic Security, 2010, pp. 3–37.

\bibitem{bib:special}
U. Rührmair, U. Schlichtmann, and W. Burleson, “Special session: How secure are PUFs really? On the reach and limits of recent PUF attacks,” in 2014 Design, Automation Test in Europe Conference Exhibition (DATE), Mar. 2014, pp. 1–4.


\bibitem{bib:gan}
J. Gan, J. Zhou, and N. Wang, \emph{A FPGA-based RO PUF with LUT-Based Self-Compare Structure and Adaptive Counter Time Period Tuning,} in 2018 IEEE International Symposium on Circuits and Systems (ISCAS), May 2018, pp. 1–5.

\bibitem{bib:wang}
Jiadong Wang, A. Cui, Mengyang Li, G. Qu, and H. Li, \emph{An ultra-low overhead LUT-based PUF for FPGA,} in 2016 IEEE Asian Hardware-Oriented Security and Trust (AsianHOST), Dec. 2016, pp. 1–6.

\bibitem{bib:ams}
F. Amsaad, A. Sherif, A. Dawoud, M. Niamat, and S. Kose, \emph{A Novel FPGA-based LFSR PUF Design for IoT and Smart Applications,} in NAECON 2018 - IEEE National Aerospace and Electronics Conference, Jul. 2018.


\bibitem{bib:cui}
W. Liu et al., “XOR-Based Low-Cost Reconfigurable PUFs for IoT Security,” ACM Trans. Embed. Comput. Syst., vol. 18, no. 3, pp. 1–21, Jun. 2019, doi: 10.1145/3274666.

\bibitem{bib:scan}
Yu Zheng, A. R. Krishna, and S. Bhunia, \emph{ScanPUF: Robust ultralow-overhead PUF using scan chain,} in 2013 18th Asia and South Pacific Design Automation Conference (ASP-DAC), Jan. 2013, pp. 626–631.

\bibitem{bib:meca}
A. R. Krishna, S. Narasimhan, X. Wang and S. Bhunia, \emph{MECCA: arobust low-overhead PUF using embedded memory array,} CHES, 2011,pp. 407-420.

\bibitem{bib:mac}
Q. Ma, C. Gu, N. Hanley, C. Wang, W. Liu and M. O’Neill, \emph{A machine learning attack resistant multi-PUF design on FPGA}, 2018 23rd Asia and South Pacific Design Automation Conf. (ASP-DAC), pp. 97-104, 2018.

\bibitem{bib:arb}
J. W. Lee, Daihyun Lim, B. Gassend, G. E. Suh, M. van Dijk, and S. Devadas, “A technique to build a secret key in integrated circuits for identification and authentication applications,” in 2004 Symposium on VLSI Circuits. Digest of Technical Papers (IEEE Cat. No.04CH37525), Jun. 2004, pp. 176–179.

\bibitem{bib:ro}
B. Gassend, D. Clarke, M. van Dijk, and S. Devadas, “Silicon physical random functions,” in Proceedings of the 9th ACM conference on Computer and communications security, New York, NY, USA, Nov. 2002, pp. 148–160.

\bibitem{bib:ro2}
W. Liu, Y. Yu, C. Wang, Y. Cui, and M. O’Neill, “RO PUF design in FPGAs with new comparison strategies,” in 2015 IEEE International Symposium on Circuits and Systems (ISCAS), May 2015, pp. 77–80, doi: 10.1109/ISCAS.2015.7168574.


\bibitem{bib:yang}
S. Yang, J. Vosatka, and S. Bhunia, “Hardware Hacking Security Education Platform (HaHa SEP v2): Enabling Hands-On Applied Research of Hardware Security Theory \& Principles,” p. 2.

\bibitem{url:ptm}
    PTM. ``Predictive Technology Model.'' 2009. [Online].  
    Available: \url{http://ptm.asu.edu/}.
    
\bibitem{Mukhopadhyay_modeling_failure}
S. Mukhopadhyay, H. Mahmoodi and K. Roy, "Modeling of failure probability and statistical design of SRAM array for yield enhancement in nanoscaled CMOS," in IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems, vol. 24, no. 12, pp. 1859-1880, Dec. 2005, doi: 10.1109/TCAD.2005.852295.

\bibitem{bib:nist_randomness}
L. E. Bassham, III, A. L. Rukhin, J. Soto, J. R. Nechvatal, M. E. Smid, E. B. Barker, S. D. Leigh, M. Levenson, M. Vangel, D. L. Banks, N. A. Heckert, J. F. Dray, and S. Vo, “SP 800-22 Rev. 1a. A Statistical Test Suite for Random and Pseudorandom Number Generators for Cryptographic Applications,” Gaithersburg, MD, United States, Tech. Rep., 2010

\bibitem{bib:clb}
"Using Look-Up Tables as Shift Registers (SRL16) in Spartan-3 Generation FPGAs", Application Note Xilinx Inc..

\bibitem{bib:mlatk}
J. Miskelly, C. Gu, Q. Ma, Y. Cui, W. Liu and M. O’Neill, "Modelling Attack Analysis of Configurable Ring Oscillator (CRO) PUF Designs," 2018 IEEE 23rd International Conference on Digital Signal Processing (DSP), Shanghai, China, 2018, pp. 1-5, doi: 10.1109/ICDSP.2018.8631638.

\bibitem{bib:tax}
T. McGrath, I. E. Bagci, Z. M. Wang, U. Roedig, and R. J. Young, “A PUF taxonomy,” Applied Physics Reviews, vol. 6, no. 1, p. 011303, Feb. 2019, doi: 10.1063/1.5079407.

\bibitem{bib:attack}
U. Rührmair, F. Sehnke, J. Sölter, G. Dror, S. Devadas, and J. Schmidhuber, Modeling Attacks on Physical Unclonable Functions. 2010, p. 249.

\bibitem{bib:iot}
A. Babaei and G. Schiele, “Physical Unclonable Functions in the Internet of Things: State of the Art and Open Challenges,” Sensors (Basel), vol. 19, no. 14, Jul. 2019, doi: 10.3390/s19143208.

\bibitem{bib:weak1}
L. Santiago et al., "Realizing strong PUF from weak PUF via neural computing," 2017 IEEE International Symposium on Defect and Fault Tolerance in VLSI and Nanotechnology Systems (DFT), Cambridge, 2017, pp. 1-6, doi: 10.1109/DFT.2017.8244433.

\bibitem{bib:weak2}
U. R ührmair, F. Sehnke, J. S ölter, G. Dror, S. Devadas, and J. ürgen Schmidhuber, “Modeling attacks on physical unclonable functions,” in Proceedings of the 17th ACM conference on Computer and communications security - CCS ’10, Chicago, Illinois, USA, 2010, p. 237, doi: 10.1145/1866307.1866335.

\end{thebibliography}


==> sections/title_page.tex <==
\begin{titlepage}

\end{titlepage}


==> sections/todo.tex <==
\begin{itemize}
    \item address reviewer feedback.
    \item improve on ML section. Will most likely need a hybrid side channel ML attack.
    \item include heat-map of average PUF response value and location. 
    \item for reliability issues discuss problems with routing. 
    \item Try to fix reliability. 
    \item purpose of ML attack was to determine if information from one FPGA can lead to revealing information about another unknown FPGA.
    \item 
    \item 
\end{itemize}

Attack on SRAM PUF. Might be applicable except you can't write to the melpuf cells. Maybe something with the power off times might be worth looking into to?
But this relies on an initial state overwriting the PUF value which simply is not happening here. 
https://eprint.iacr.org/2015/148.pdf

